The conclusion that metamaterials could have negative mass is a consequence of improper constitutive characterisation

The concept of "effective mass" is frequently used for the simplification of complex lumped parameter systems (discrete dynamical systems) as well as materials that have complicated microstructural features. From the perspective of wave propagation, it is claimed that for some bodies described as metamaterials, the corresponding "effective mass" can be frequency dependent, negative or it may not even be a scalar quantity. The procedure has even led some authors to suggest that Newton's second law needs to be modified within the context of classical continuum mechanics. Such absurd physical conclusions are a consequence of appealing to the notion of "effective mass" with a preconception for the constitutive structure of the metamaterial and using a correct mathematical procedure. We show that such unreasonable physical conclusions would not arise if we were to use the appropriate "effective constitutive relation" for the metamaterial, rather than use the concept of "effective mass" with an incorrect predetermined constitutive relation.

==> integral-transforms.tex <==
\newcommand{\FourierTransform}[1]{\fouriertransforms \left[#1\right]}
\newcommand{\InverseFourierTransform}[1]{\inverse{\fouriertransforms} \left[#1\right]}


==> text/discrete-versus-continuous-body.tex <==

\todo[inline]{I would prefer to do the following analysis for the monoatomic one-dimensional lattice model in another paper. This issue is not related to the negative mass only.}


\section{Discrete versus continuous}
\label{sec:discr-vers-cont}

Concerning the dispersion relation, there are two problems.
\begin{enumerate}
\item We have a discrete system (classical one-dimensional lattice model), and we want to design a continuous system that has the same dispersion relation as the discrete one.
\item We have a continuous system (classical one-dimensional linearised elasticity), and we want to design a discrete lattice system that has the same dispersion relation as the continuous one. 
\end{enumerate}

\subsection{Infinite chain}
\label{sec:infinite-chain}

We want find dispersion relation for the one-dimensional monoatomic lattice model described by the system of equations 
\begin{equation}
  \label{eq:13}
  \ddd{\uj{j}}{t} - \cdiscrete^2 \left(\uj{j+1} - 2 \uj{j} + \uj{j-1} \right) = 0, 
\end{equation}
wherein the masses are at fixed distances $h$ apart. (The notation is clear $\uj{j} =_{\bydefinition}u(jh)$.) The task is to find a relation between the discrete system~\eqref{eq:13} and the continuous system
\begin{equation}
  \label{eq:14}
  \ppd{u}{t} - \ccontinuous^2 \ppd{u}{x} = 0,
\end{equation}
or between the discrete system
\begin{equation}
  \label{eq:48}
  \ddd{\uj{j}}{t} - \cdiscrete^2 \sum_{k=-\infty}^{\infty} \tensor{\tensorc{D}}{_j_k}\uj{j} = 0
\end{equation}
and the continuous system
\begin{equation}
  \label{eq:49}
  \ppd{u}{t} - \ccontinuous^2 \mathcal{L}(u) = 0,
\end{equation}
where $\tensorq{D}$ is an infinite matrix and $\mathcal{L}$ is a linear operator. (Preferably constructed in such a way that it ``includes'' the second derivative operator.)

\subsubsection{Identification of continuous system that has the same dispersion relation as the discrete one}
\label{sec:ident-cont-syst}
First we want to find the dispersion relation for the discrete system~\eqref{eq:13}. We recall that the (continuous) Fourier transform of $g\colon\, \vec{x} \in \R^n \mapsto \R$ and the corresponding inverse Fourier transform are defined by the formulae
\begin{subequations}
  \label{eq:68}
  \begin{align}
    \label{eq:11}
    \fouriertransform{g(\vec{x})}{\vec{\xi}}
    &=_{\bydefinition}
      \frac{1}{\left(2 \pi \right)^{\frac{n}{2}}}
      \int_{\vec{x} \in \R^n}
      g(\vec{x})
      \,
      \exponential{\iunit \vectordot{\vec{x}}{\vec{\xi}}}
      \,
      \cvolumee_{\vec{x}}
      , \\
    \label{eq:12}
    \inversefouriertransform{g(\vec{\xi})}{\vec{x}}
    &=_{\bydefinition}
      \frac{1}{\left(2 \pi \right)^{\frac{n}{2}}}
      \int_{\vec{\xi} \in \R^n}
      g(\vec{\xi})
      \,
      \exponential{-\iunit \vectordot{\vec{\xi}}{\vec{x}}}
      \,
      \cvolumee_{\vec{\xi}}
      .
  \end{align}
\end{subequations}
Here we use the convention used in~\cite[Theorem 10]{sneddon.in:fourier}. We will be using the Fourier transformation only for $n=1$. The definition of convolution is then
\begin{equation}
  \label{eq:66}
  (\convolution{f}{g})(x)
  =_{\bydefinition}
  \frac{1}{\sqrt{2 \pi}}
  \int_{\eta = -\infty}^{+\infty}
  f(x-\eta)
  g(\eta)
  \,
  \diff \eta,
\end{equation}
see~\cite[Section 3.6]{sneddon.in:fourier}, and with this definition of Fourier transform and convolution we obtain the convolution theorem in the form
\begin{equation}
  \label{eq:67}
  \fouriertransform{(\convolution{f}{g})(x)}{\xi}
  =
  \fouriertransform{f(x)}{\xi}
  \fouriertransform{g(x)}{\xi}
  ,
\end{equation}
see~\cite[Theorem 12]{sneddon.in:fourier}. We also recall that under the convention~\eqref{eq:68} we have
\begin{equation}
  \label{eq:15}
  \fouriertransform{\diracdelta_0 \left(x\right)}{\xi}
  =
  \frac{1}{\sqrt{2 \pi}},
\end{equation}
where $\diracdelta_0 \left(x\right)$ denotes the Dirac delta function centred at $x=0$. Furthermore, we also have the sampling/sifting property
\begin{equation}
  \label{eq:16}
  f(x - \xi) = \sqrt{2\pi} \left(\convolution{\diracdelta_\xi}{f} \right)(x),
\end{equation}
indeed,
\begin{equation}
  \label{eq:17}
  \sqrt{2\pi} \left(\convolution{\diracdelta_\xi}{f} \right)(x)
  =
  \int_{\eta = -\infty}^{+\infty}
  \diracdelta_\xi (x-\eta)
  f(\eta)
  \,
  \diff \eta
  =
  \int_{\eta = -\infty}^{+\infty}
  \diracdelta_0 (x-\eta-\xi)
  f(\eta)
  \,
  \diff \eta
  =
  \int_{\eta = -\infty}^{+\infty}
  \diracdelta_0 (\left(x-\xi\right)-\eta)
  f(\eta)
  \,
  \diff \eta
  =
  f(x - \xi).
\end{equation}
Using the properties of the Dirac delta function, we see that the discrete system~\eqref{eq:13} can be rewritten as
\begin{equation}
  \label{eq:18}
  \ddd{}{t} \convolution{\diracdelta}{u} - \cdiscrete^2 \convolution{\left( \diracdelta_{h} - 2 \diracdelta + \diracdelta_{-h} \right)} u = 0.
\end{equation}
\todo[inline]{This is not well written. This is the equation for all $x$, we should use only sampling points $x_j$. Product $\diracdelta_{(j+n)h} u$ will be better/more instructive.}%
(Here we emphasise that the Dirac delta function is a function of the $x$ variable.) Equation~\eqref{eq:18} indicates that~\eqref{eq:13} can be interpreted as sampling of a continuous function at points $x_j=jh$. Now we apply Fourier transform to~\eqref{eq:18}, and we use the convolution theorem~\eqref{eq:67}. This yields
\begin{equation}
  \label{eq:20}
  \ddd{}{t} \FourierTransform{\diracdelta}\FourierTransform{u} - \cdiscrete^2 \FourierTransform{\left( \diracdelta_{h} - 2 \diracdelta + \diracdelta_{-h} \right)} \FourierTransform{u} = 0
\end{equation}
The shift property of the Fourier transformation yields
\begin{equation}
  \label{eq:19}
  \fouriertransform{\diracdelta_{\pm h}(x)}{\xi}
  =
  \fouriertransform{\diracdelta_{jh}(x \mp h)}{\xi}
  =
  \exponential{\pm \iunit  h \xi}
  \fouriertransform{\diracdelta(x)}{\xi}
  =
  \frac{\exponential{\pm \iunit  h \xi}}{\sqrt{2 \pi}}  
  ,
\end{equation}
hence we can further rewrite~\eqref{eq:20} as
\begin{equation}
  \label{eq:21}
  \left(
    \ddd{}{t}
    -
    \cdiscrete^2
    \left(
      \exponential{\iunit  h \xi}
      -
      2
      +
      \exponential{-\iunit  h \xi}
    \right)
  \right)
  \FourierTransform{u}
  =
  0
  ,
\end{equation}
which yields
\begin{equation}
  \label{eq:22}
  \left(
    \ddd{}{t}
    +
    2
    \cdiscrete^2
    \left(
      1
      -
      \cos \left( h \xi \right)
    \right)
  \right)
  \FourierTransform{u}
  =
  0
  .  
\end{equation}
If we do yet another Fourier transformation, now with respect to the time variable $t \leftrightarrow \omega$, then we get
\begin{equation}
  \label{eq:23}
  \left(
    -
    \omega^2
    +
    2
    \cdiscrete^2
    \left(
      1
      -
      \cos \left( h \xi \right)
    \right)
  \right)
  \FourierTransform{\FourierTransform{u}}
  =
  0
  ,
\end{equation}
which yields the standard dispersion relation
\begin{equation}
  \label{eq:24}
  \omega^2
  =
  2
  \cdiscrete^2
  \left(
    1
    -
    \cos \left( h \xi \right)
  \right)
  .
\end{equation}
Note that this can be also rewritten as
\begin{equation}
  \label{eq:25}
  \omega^2
  =
  4
  \cdiscrete^2
  \sin^2 \left( \frac{h \xi}{2} \right).
\end{equation}

If we now want to see the continuous counterpart of~\eqref{eq:22} back in the physical space and preferably with some differential operators instead of sampling operators, we can proceed as follows. The standard approach is based on the Taylor series approximation
\begin{equation}
  \label{eq:26}
  1
  -
  \cos \left( h \xi \right)
  \approx
  \frac{h^2 \xi^2}{2}
  -
  \frac{h^4 \xi^4}{24}
  +
  \cdots,
\end{equation}
which yields the approximation of~\eqref{eq:22} as
\begin{equation}
  \label{eq:27}
  \left(
    \ddd{}{t}
    +
    \cdiscrete^2
    \left(
      h^2 \xi^2
      -
      \frac{h^4 \xi^4}{12}
      +
      \cdots
    \right)
  \right)
  \FourierTransform{u}
  =
  0
  .
\end{equation}
Using the standard formula for the Fourier transform of the derivative,
\begin{equation}
  \label{eq:28}
  \FourierTransform{\ppd{u}{x}} = - \xi^2   \FourierTransform{u}.
\end{equation}
we can finally rewrite~\eqref{eq:27} in the physical space as
\begin{equation}
  \label{eq:29}
  \left(
    \ddd{}{t}
    -
    \cdiscrete^2
    \left(
      h^2 \ppd{}{x}
      +
      \frac{h^4}{12} \pd{^4}{x^4}
      +
      \cdots
    \right)
  \right)
  u
  =
  0
  .
\end{equation}
The is approximation used in various works. \todo[inline]{Give references.}
Another possibility is to start in the physical space and use the symbolic manipulation
\begin{equation}
  \label{eq:30}
  u(x + h)
  =
  \exponential{h\pd{}{x}} u(x),
\end{equation}
which is just an obscure way how to write the Taylor expansion
\begin{equation}
  \label{eq:31}
  u(x + h)
  =
  \sum_{j=0}^{+ \infty}
  \frac{1}{j!}
  \pd{^ju}{x^j}
  h^j
  .
\end{equation}
Using the translation operator introduced in~\eqref{eq:30}, we see that~\eqref{eq:13} can be rewritten as
\begin{equation}
  \label{eq:32}
  \ddd{u}{t} - \cdiscrete^2 \left(\exponential{h\pd{}{x}} - 2  + \exponential{-h\pd{}{x}}\right)u = 0.
\end{equation}
This can be further manipulated into the form
\begin{equation}
  \label{eq:33}
  \ddd{u}{t} - 4 \cdiscrete^2 \sinh^2 \left(\frac{h}{2} \pd{}{x} \right) u = 0.
\end{equation}
Using formally the Pad\'e approximation for $\sinh^2$ one can finally write
\begin{equation}
  \label{eq:34}
  \sinh^2 \left(\frac{h}{2} \pd{}{x} \right)
  =
  \frac{ \left( \frac{h}{2} \pd{}{x} \right)^2}{ 1 - \frac{\left(\frac{h}{2} \pd{}{x} \right)^2}{3}},
\end{equation}
which upon substitution into~\eqref{eq:33} leads to
\begin{equation}
  \label{eq:35}
  \left(\left( 1 - \frac{h^2}{12} \ppd{}{x} \right) \ddd{}{t} - \cdiscrete^2 h^2 \ppd{}{x} \right) u = 0.
\end{equation}
This is yet another popular approach to ``continualisation'' of the discrete lattice system, see~\cite{challamel.n.picandet.v.ea:revisiting} and references therein. It however seems that one possibility that yields \emph{exact} continuous counterpart of~\eqref{eq:13} has been missed in the literature. We return to~\eqref{eq:22} and we insert the desired second derivative into the equation
\begin{equation}
  \label{eq:36}
  \ddd{}{t}
  \FourierTransform{u}
  +
  2
  \cdiscrete^2
  \frac{
    1
    -
    \cos \left( h \xi \right)
  }{\xi^2}
  \xi^2
  \FourierTransform{u}
  =
  0.
\end{equation}
This gives
\begin{equation}
  \label{eq:37}
    \ddd{}{t}
  \FourierTransform{u}
  -
  2
  \cdiscrete^2
  \frac{
    1
    -
    \cos \left( h \xi \right)
  }{\xi^2}
  \FourierTransform{\ppd{}{x}}
  =
  0.
\end{equation}
We can further write
\begin{equation}
  \label{eq:38}
  \ddd{}{t}
  \FourierTransform{u}
  -
  \cdiscrete^2
  \FourierTransform{
    \InverseFourierTransform{
      2
      \frac{
        1
        -
        \cos \left( h \xi \right)
      }{\xi^2}
    }
  }
  \FourierTransform{\ppd{}{x}}
  =
  0
  ,
\end{equation}
and using the convolution theorem the equation reduces to
\begin{equation}
  \label{eq:39}
  \ddd{}{t}
  \FourierTransform{u}
  -
  \cdiscrete^2
  \FourierTransform{
    \convolution{
    \InverseFourierTransform{
      2
      \frac{
        1
        -
        \cos \left( h \xi \right)
      }{\xi^2}
    }
  }
  {
    \ppd{u}{x}
  }
  }
  =
  0
  ,
\end{equation}
which upon the transformation to the physical space yields
\begin{equation}
  \label{eq:40}
  \ppd{u}{t}
  -
  \cdiscrete^2
  \convolution{
    \InverseFourierTransform{
      2
      \frac{
        1
        -
        \cos \left( h \xi \right)
      }{\xi^2}
    }
  }
  {
    \ppd{u}{x}
  }
  =
  0.
\end{equation}
If we manage to find a nice formula for the preimage of the function
$
2
\frac{
  1
  -
  \cos \left( h \xi \right)
}{\xi^2}
$,
then we are done. Fortunately, this is easy to do. We know the Fourier transform of the unit triangle function
\begin{equation}
  \label{eq:41}
  \UnitTriangle(x)
  =_\bydefinition
  \begin{cases}
  0,& x \in (-\infty, -1), \\
  x+1, & x \in [-1, 0], \\
  -x+1, & x \in (0, 1], \\
    0, & x \in (1, +\infty).
  \end{cases}
\end{equation}
(Vertically symmetric isosceles triangle centered at the origin with base $[-1,1]$ and height $1$.) Using our convention for the Fourier transform we have
\begin{equation}
  \label{eq:42}
  \fouriertransform{\UnitTriangle(x)}{\xi} = \frac{1}{\sqrt{2 \pi}} \sinc^2 \left( \frac{\xi}{2} \right),
\end{equation}
where $\sinc x =_{\bydefinition} \frac{\sin x}{x}$. This implies that
\begin{equation}
  \label{eq:43}
  \fouriertransform{\UnitTriangle \left( \frac{x}{h} \right)}{\xi}
  =
  \frac{h}{\sqrt{2 \pi}} \sinc^2 \left( \frac{h \xi}{2} \right).
\end{equation}
Making use of~\eqref{eq:43} we see that
\begin{multline}
  \label{eq:44}
      \InverseFourierTransform{
      2
      \frac{
        1
        -
        \cos \left( h \xi \right)
      }{\xi^2}
    }
    =
    \InverseFourierTransform{
      4
      \frac{
        \sin^2 \left( \frac{h \xi}{2} \right)
      }{\xi^2}
    }
    =
    h^2
    \InverseFourierTransform{
      \frac{
        \sin^2 \left( \frac{h \xi}{2} \right)
      }
      {
        \left( \frac{h \xi}{2} \right)^2
      }
    }
    \\
    =
    h
    \sqrt{2 \pi}
    \InverseFourierTransform{
      \frac{h}{\sqrt{2 \pi}}
      \frac{
        \sin^2 \left( \frac{h \xi}{2} \right)
      }
      {
        \left( \frac{h \xi}{2} \right)^2
      }
    }
    =
     h
    \sqrt{2 \pi}
    \InverseFourierTransform{
      \frac{h}{\sqrt{2 \pi}}
      \sinc^2 \left( \frac{h \xi}{2} \right)
    }
    =
    h
    \sqrt{2 \pi}
    \UnitTriangle \left( \frac{x}{h} \right)
    ,
  \end{multline}
  and consequently~\eqref{eq:40} reduces to
  \begin{equation}
    \label{eq:45}
    \ppd{u}{t}
    -
    \cdiscrete^2 h^2
    \convolution{
    \frac{\sqrt{2 \pi}}{h}
    \UnitTriangle \left( \frac{x}{h} \right)
    }
    {
      \ppd{u}{x}
    }
    =
    0.    
  \end{equation}
  Since for $h \to 0$ we have
  \begin{equation}
    \label{eq:46}
    \frac{1}{h}
    \UnitTriangle \left( \frac{x}{h} \right)
    \to \diracdelta(x),
  \end{equation}
  we see that we can make approximation
  $
  \frac{1}{h}
  \UnitTriangle \left( \frac{x}{h} \right)
  \approx \diracdelta (x)
  $,
  which means that for small $h$ we can formally approximate the \emph{exact} equation~\eqref{eq:45} as
  \begin{equation}
    \label{eq:47}
        \ppd{u}{t}
    -
    \cdiscrete^2 h^2
    \ppd{u}{x}
    =
    0
    ,
  \end{equation}
  which is the standard naive countinuous counterpart of~\eqref{eq:13}.
  
\todo[inline]{We should be using semidiscrete (bandwidth limited) Fourier transform.}
\todo[inline]{Explain how to deal with density versus mass and stiffness scaling. This gives the right $h^2$ factor.}

\subsubsection{Identification of discrete system that has the same dispersion relation as the continuous one}
\label{sec:ident-discr-syst}
Now we want to do the opposite. We claim that the continuous system is the ground truth, and we want to identify the discrete system of type~\eqref{eq:48} that has the same dispersion relation as the continuous one. The discrete system~\eqref{eq:13} can be rewritten as
\begin{equation}
  \label{eq:50}
    \ddd{}{t}
  \begin{bmatrix}
    \vdots \\
    u_{-2} \\
    u_{-1} \\
    u_0 \\
    u_1 \\
    u_2 \\
    \vdots
  \end{bmatrix}
  -
  \cdiscrete^2
  \begin{bmatrix}
    \ddots & \vdots & \vdots & \vdots & \vdots & \vdots & \reflectbox{$\ddots$} \\
    \cdots & c_0 & c_1 & c_2 & c_3 & c_4 & \cdots \\
    \cdots & c_1 & c_0 & c_1 & c_2 & c_3 & \cdots \\
    \cdots & c_2 & c_1 & c_0 & c_1 & c_2 & \cdots \\
    \cdots & c_3 & c_2 & c_1 & c_0 & c_1 & \cdots \\
    \cdots & c_4 & c_3 & c_2 & c_1 & c_0 & \cdots \\
    \reflectbox{$\ddots$} & \vdots & \vdots & \vdots & \vdots & \vdots & \ddots
  \end{bmatrix}
  \begin{bmatrix}
    \vdots \\
    u_{-2} \\
    u_{-1} \\
    u_0 \\
    u_1 \\
    u_2 \\
    \vdots
  \end{bmatrix}
  =
  0.
\end{equation}
In the standard setting we would have
\begin{equation}
  \label{eq:51}
  c_0 = -2, \qquad c_1 = 1,
\end{equation}
and all other entries will be equal to zero.

\todo[inline]{The class of operators represented by the doubly infinite matrix as in~\eqref{eq:50} is referred to as the Laurent operators, see \cite{gohberg.i.goldberg.s.ea:basic}. It is time to read the relevant literature. See also~\cite{reichel.l.trefethen.ln:eigenvalues}.}

If written in indices, the equation~\eqref{eq:50} reads
\begin{equation}
  \label{eq:72}
  \ddd{u_j}{t}
  -
  \cdiscrete^2
  \sum_{m=-\infty}^{+ \infty} c_{m-j}u_m
  =
  0.
\end{equation}
(With the property $c_i = c_{-i}$.) Now we use the apparatus of semidiscrete Fourier transform. We define forward transform from the discrete physical space---sampling of a function $u$ at the corresponding points, $u_j = u(jh)$---to the wave number space as
\begin{equation}
  \label{eq:73}
  \FourierTransform{u} =_{\bydefinition}
  h
  \sum_{j= - \infty}^{+ \infty}
  u_j
  \exponential{- \iunit \xi x_j},
\end{equation}
where $x_j = jh$, $h$ being the distance between the neighboring points and $\xi$, the wave number, being restricted to $\xi \in \left[ - \frac{\pi}{h}, \frac{\pi}{h} \right]$. (In physics this is called Brillouin zone, in mathematics this is the way how to avoid the aliasing phenomenon.) The inverse transformation is
\begin{equation}
  \label{eq:74}
  u_j
  =
  \frac{1}{2\pi}
  \int_{\xi = - \frac{\pi}{h}}^{\frac{\pi}{h}}
  \FourierTransform{u}
  \exponential{\iunit \xi x_j}
  \,
  \diff \xi.
\end{equation}
The convolution is defined as
\begin{equation}
  \label{eq:75}
  \tensor{
    \left( \convolution{u}{v} \right)
  }{_k}
  =_{\bydefinition}
  h
  \sum_{j=-\infty}^{+\infty}
  u_{k-j}v_j
\end{equation}
and with these definitions we have
\begin{equation}
  \label{eq:76}
  \FourierTransform{\convolution{u}{v}}
  =
  \FourierTransform{u}\FourierTransform{v}.
\end{equation}
Consequently, the Fourier image of~\eqref{eq:72} reads
\begin{equation}
  \label{eq:77}
  \ddd{\FourierTransform{u}}{t}
  -
  \cdiscrete^2
  \FourierTransform{c}
  \FourierTransform{u}
  =
  0
  .
\end{equation}
(We have formally multiplied~\eqref{eq:72} by $h\exponential{- \iunit \xi x_j}$, and then we have summed all the equations with respect to $j$, that is $  \sum_{j= - \infty}^{+ \infty} \left( \cdots \right) \exponential{- \iunit \xi x_j}$.) Here the symbol $c$ denotes the vector
\begin{equation}
  \label{eq:78}
  c
  =_{\bydefinition}
  \begin{bmatrix}
     \vdots \\ c_2 \\ c_1 \\ c_0 \\ c_1 \\ c_2 \\ \vdots
  \end{bmatrix}
\end{equation}
Thus if we want to preserve the standard dispersion relation for the equation~\eqref{eq:14}, we must fix
\begin{equation}
  \label{eq:79}
  \fouriertransform{c}{\xi}
  =
  \xi^2
  ,
\end{equation}
which means that the vector $c$ in the physical space is given as
\begin{equation}
  \label{eq:80}
  c
  =
  \begin{bmatrix}
    c_j
  \end{bmatrix}_{j=-\infty}^{+\infty}
  =
  \begin{bmatrix}
    -
    \frac{1}{2\pi}
    \int_{\xi = - \frac{\pi}{h}}^{\frac{\pi}{h}}
    \xi^2
    \exponential{\iunit \xi x_j}
    \,
    \diff \xi
  \end{bmatrix}_{j=-\infty}^{+\infty},
\end{equation}
which is the inverse semidiscrete Fourier transform of function $-\xi^2$. Evaluating the integral yields
\begin{equation}
  \label{eq:81}
  c_j
  =
  \frac{2 \left(-1\right)^{j+1}}{j^2h^3}.
\end{equation}
\todo[inline]{Factor $\frac{1}{h}$ is missing?}
\todo[inline]{This seems to be known fact in the numerical community, they know that the spectral methods are non-dispersive. Can we interpret this as pairwise interactions with distant neighbors?}

\subsection{Finite length, periodic boundary conditions}
\label{sec:peri-bound-cond}
\cite{chao.c:remark,rojo.o.rojo.h:some}
\todo[inline]{This is a mess. I am mixing several conventions.}
We want find dispersion relation for the one-dimensional monoatomic lattice model described by the system of equations 
\begin{equation}
  \label{eq:1}
  \ddd{\uj{j}}{t} - \cdiscrete^2 \left(\uj{j+1} - 2 \uj{j} + \uj{j-1} \right) = 0, 
\end{equation}
where $j=-N, \dots, -1, 0, 1, \dots, N$. We have $2N+1$ masses, the length of the whole chain is $L$, the masses are distributed equidistantly, thus the distance between the masses is
\begin{equation}
  \label{eq:2}
  h = \frac{L}{2N}.
\end{equation}
Next we do the same for the continuous model described by the partial differential equation
\begin{equation}
  \label{eq:3}
  \ppd{u}{t} - \ccontinuous^2 \ppd{u}{x} = 0.
\end{equation}
The partial differential equation ought to be solved in the spatial domain $\left(- \frac{L}{2}, \frac{L}{2} \right)$, the system of ordinary differential equations ought to be solved for $2N+1$ functions $\left\{ \uj{j} \right\}_{j=-N}^{N}$. In both case we search for periodic solutions with period $L$, that is in the continuous case we want
\begin{equation}
  \label{eq:5}
  u(x)  = u(x+L)
\end{equation}
while in the discrete case we in~\eqref{eq:1} formally set 
\begin{subequations}
  \label{eq:6}
  \begin{align}
    \label{eq:52}
    \uj{N+1} &= \uj{-N}, \\
    \label{eq:53}
    \uj{-N-1} &= \uj{N}.
  \end{align}
\end{subequations}
The notation is clear $\uj{j} =_{\bydefinition}u(jh)$.


The continuous model is easy to deal with. If look for the solution in the form
\begin{equation}
  \label{eq:4}
   u(x, t) = \sum_{j=-\infty}^{+\infty} \widehat{u} \exponential{\iunit \frac{2 \pi}{L} j x}. 
 \end{equation}
 (This is the same as if we write $\exponential{\iunit \left( \xi x - \Omega t\right)}$, and we are interested in the proper wavenumber $\xi$, we already know that $\xi_j = \frac{2 \pi}{L} j$. The wavenumbers are in the periodic case discrete and so are the frequencies.)
The equation then reduces to
 \begin{equation}
   \label{eq:4}
   \left[ \ddd{}{t} + \ccontinuous^2 \left( \frac{2 \pi}{L} j \right)^2 \right] \widehat{u} = 0,
 \end{equation}
 which means that the dispersion relation reads
 \begin{equation}
   \label{eq:9}
   \Omega_j^2 = \ccontinuous^2 \left( \frac{2 \pi}{L} j \right)^2.
 \end{equation}
 The dispersion relation thus reads
 \begin{equation}
   \label{eq:54}
   \Omega_j^2 = \ccontinuous^2 \xi_j^2.
 \end{equation}

 We note that the system~\eqref{eq:1} can be rewritten in the matrix form
\begin{equation}
  \label{eq:7}
  \ddd{\vec{u}}{t}
  -
  \cdiscrete^2
  \tensorq{D}
  \vec{u}
  =
  0,
\end{equation}
where $\tensorq{D}$ represents the discrete counterpart of the second spatial derivative. The matrix representing the second derivative/interactions between equally spaced masses should have the structure of the symmetric circulant matrix. (The interaction with the nearest neighbour to the left should be the same as the interaction with the nearest neighbour to the right and and so forth for more distant neighbours.) For example for $N=3$ we should deal with the matrix
\begin{equation}
  \label{eq:55}
  \ddd{}{t}
  \begin{bmatrix}
    \uj{-3} \\
    \uj{-2} \\
    \uj{-1} \\
    \uj{0} \\
    \uj{1} \\
    \uj{2} \\
    \uj{3}
  \end{bmatrix}
  -
  \cdiscrete^2
  \begin{bmatrix}
    c_0 & c_1 & c_2 & c_3 & c_3 & c_2 & c_1 \\
    c_1 & c_0 & c_1 & c_2 & c_3 & c_3 & c_2 \\
    c_2 & c_1 & c_0 & c_1 & c_2 & c_3 & c_3 \\
    c_3 & c_2 & c_1 & c_0 & c_1 & c_2 & c_3 \\
    c_3 & c_3 & c_2 & c_1 & c_0 & c_1 & c_2 \\
    c_2 & c_3 & c_3 & c_2 & c_1 & c_0 & c_1 \\
    c_1 & c_2 & c_3 & c_3 & c_2 & c_1 & c_0 \\
  \end{bmatrix}
  \begin{bmatrix}
    \uj{-3} \\
    \uj{-2} \\
    \uj{-1} \\
    \uj{0} \\
    \uj{1} \\
    \uj{2} \\
    \uj{3}
  \end{bmatrix}
  .
\end{equation}
In particular, for the choice
\begin{equation}
  \label{eq:51}
  c_0 = -2, \qquad c_1 = 1,
\end{equation}
and all other entries being equal to zero we get
\begin{equation}
  \label{eq:56}
   \ddd{}{t}
  \begin{bmatrix}
    \uj{-3} \\
    \uj{-2} \\
    \uj{-1} \\
    \uj{0} \\
    \uj{1} \\
    \uj{2} \\
    \uj{3}
  \end{bmatrix}
  -
  \cdiscrete^2
  \begin{bmatrix}
    -2 & 1 & 0 & 0 & 0 & 0 & 1 \\
    1 & -2 & 1 & 0 & 0 & 0 & 0 \\
    0 & 1 & -2 & 1 & 0 & 0 & 0 \\
    0 & 0 & 1 & -2 & 1 & 0 & 0 \\
    0 & 0 & 0 & 1 & -2 & 1 & 0 \\
    0 & 0 & 0 & 0 & 1 & -2 & 1 \\
    1 & 0 & 0 & 0 & 0 & 1 & -2 \\
  \end{bmatrix}
  \begin{bmatrix}
    \uj{-3} \\
    \uj{-2} \\
    \uj{-1} \\
    \uj{0} \\
    \uj{1} \\
    \uj{2} \\
    \uj{3}
  \end{bmatrix}
  .
\end{equation}
This is the standard second order differentiation matrix for finite differences discretisation of the second derivative. (Please note the ones at the top right corner and the bottom left corner.)

The circulant matrices are easy to deal with in terms of discrete Fourier transform, see, for example, \cite{davis.pj:circulant} or \cite{golub.gh.van-loan.cf:matrix}, or the review paper \cite{olson.bj.shaw.sw.ea:circulant}. We introduce the notation $\omega_n$ for the $n$-th complex root of unity, that is
\begin{equation}
  \label{eq:57}
  \omega_n =_{\bydefinition} \exponential{\frac{2 \pi \iunit}{n}},
\end{equation}
ans we fix $n$ to be equal to the row/column dimension of the square matrix. In our case we set
\begin{equation}
  \label{eq:63}
  n = 2N+1.
\end{equation}
Now we observe what happens if we apply the matrix to the vector
\begin{equation}
  \label{eq:58}
    \vec{w}_k
    =_{\bydefinition}
    \begin{bmatrix}
      \omega_n^{-N k} \\
      \omega_n^{\left(-N+1\right)k} \\
      \vdots \\
      \omega_n^{-2k} \\
      \omega_n^{-k} \\
      \omega_n^{0} \\
      \omega_n^{k} \\
      \omega_n^{2k} \\
      \vdots \\
      \omega_n^{\left(N-1\right)k} \\
      \omega_n^{Nk},
  \end{bmatrix}
\end{equation}
where $k =-N, \dots, 0, \dots, N$. (We have as many $k$ as the row/column dimension of the corresponding square matrix.) The upper index in $\omega_n^{\left(N-1\right)k}$ is the exponent, that is $\omega_n^{\left(N-1\right)k}= \exponential{\frac{2 \pi \iunit}{n} \left(N-1\right)k}$, and we observe that
\begin{equation}
  \label{eq:59}
  \omega_n^{j\pm n} = \omega_n^{j},
\end{equation}
which the key periodicity property. Using this property, we see that
\begin{multline}
  \label{eq:61}
    \begin{bmatrix}
    c_0 & c_1 & c_2 & c_3 & c_3 & c_2 & c_1 \\
    c_1 & c_0 & c_1 & c_2 & c_3 & c_3 & c_2 \\
    c_2 & c_1 & c_0 & c_1 & c_2 & c_3 & c_3 \\
    c_3 & c_2 & c_1 & c_0 & c_1 & c_2 & c_3 \\
    c_3 & c_3 & c_2 & c_1 & c_0 & c_1 & c_2 \\
    c_2 & c_3 & c_3 & c_2 & c_1 & c_0 & c_1 \\
    c_1 & c_2 & c_3 & c_3 & c_2 & c_1 & c_0 \\
  \end{bmatrix}
  \begin{bmatrix}
      \omega_n^{-3k} \\
      \omega_n^{-2k} \\
      \omega_n^{-k} \\
      \omega_n^{0} \\
      \omega_n^{k} \\
      \omega_n^{2k} \\
      \omega_n^{3k}
  \end{bmatrix}
  =
  \begin{bmatrix}
    c_0 \omega_n^{-3k}
    +
    c_1 \omega_n^{-2k}
    +
    c_2 \omega_n^{-k}
    +
    c_3 \omega_n^{0}
    +
    c_3 \omega_n^{k}
    +
    c_2 \omega_n^{2k}
    +
    c_1 \omega_n^{3k}
    \\
    c_1 \omega_n^{-3k}
    +
    c_0 \omega_n^{-2k}
    +
    c_1 \omega_n^{-k}
    +
    c_2 \omega_n^{0}
    +
    c_3 \omega_n^{k}
    +
    c_3 \omega_n^{2k}
    +
    c_2 \omega_n^{3k}
    \\
    \vdots
    \\
    \vdots
    \\
    \vdots
    \\
    \vdots
    \\
    c_1 \omega_n^{-3k}
    +
    c_2 \omega_n^{-2k}
    +
    c_3 \omega_n^{-k}
    +
    c_3 \omega_n^{0}
    +
    c_2 \omega_n^{k}
    +
    c_1 \omega_n^{2k}
    +
    c_0 \omega_n^{3k}
  \end{bmatrix}
  \\
  =
  \left(
  c_0 
  +
  c_1 \omega_n^{k}
  +
  c_2 \omega_n^{2k}
  +
  c_3 \omega_n^{3k}
  +
  c_3 \omega_n^{-3k}
  +
  c_2 \omega_n^{-2k}
  +
  c_1 \omega_n^{-k}
\right)
 \begin{bmatrix}
      \omega_n^{-3k} \\
      \omega_n^{-2k} \\
      \omega_n^{-k} \\
      \omega_n^{0} \\
      \omega_n^{k} \\
      \omega_n^{2k} \\
      \omega_n^{3k}
 \end{bmatrix}
 =
 \left(
   c_0
   +
   c_1
   \left(
     \omega_n^{k}
     +
     \omega_n^{-k}
   \right)
   +
   c_2
   \left(
     \omega_n^{2k}
     +
     \omega_n^{-2k}
   \right)
   +
   c_3
   \left(
     \omega_n^{3k}
     +
     \omega_n^{-3k}
   \right)
 \right)
 \begin{bmatrix}
      \omega_n^{-3k} \\
      \omega_n^{-2k} \\
      \omega_n^{-k} \\
      \omega_n^{0} \\
      \omega_n^{k} \\
      \omega_n^{2k} \\
      \omega_n^{3k}
 \end{bmatrix}
 \\
 =
 \left(
   c_0
   +
   2
   c_1
   \cos \left( \frac{2 \pi}{n} k\right)
   +
   2
   c_2
   \cos \left( \frac{2 \pi}{n} 2 k\right)
   +
   2
   c_3
   \cos \left( \frac{2 \pi}{n} 3 k\right)
 \right)
 \begin{bmatrix}
      \omega_n^{-3k} \\
      \omega_n^{-2k} \\
      \omega_n^{-k} \\
      \omega_n^{0} \\
      \omega_n^{k} \\
      \omega_n^{2k} \\
      \omega_n^{3k}
 \end{bmatrix}
 .
\end{multline}
Consequently, we see that every vector $\vec{w}_k$, $k=-N, \dots, 0, \dots,  N$, is an eigenvector of the corresponding circulant matrix. (We note that the eigenvectors of \emph{any} circulant matrix have the form~\eqref{eq:58}, the particular values of matrix elements $\left\{c_i \right\}_{i=0}^N$ are irrelevant.) The corresponding eigenvalues are real, and are given by the formula
\begin{equation}
  \label{eq:62}
  \lambda_k
  =
  c_0
  +
  2
  \sum_{m=1}^N
  c_m
  \cos \left( \frac{2 \pi}{n} m k\right).
\end{equation}
(This is a known result, see, for example, \cite[Corollary 17]{olson.bj.shaw.sw.ea:circulant}.)  We see that the eigenvalues are degenerate in the sense that $\lambda_{-k} = \lambda_{k}$, only $\lambda_0$ is non-degenerate. If we use~\eqref{eq:51} then~\eqref{eq:62} gives
\begin{equation}
  \label{eq:8}
  \lambda_k
  =
  -
  2
  +
  2
  \cos \left( \frac{2 \pi}{n} k\right),
\end{equation}
which yields the classical formula known from the theory of finite differences
\begin{equation}
  \label{eq:10}
  \lambda_k = -4 \sin^2 \left( \frac{\pi}{n} k \right).
\end{equation}
Finally, the eigenvectors corresponding to the degenerate eigenvalues can be rearranged in such a way that they are real. Indeed, we can set
\begin{subequations}
  \label{eq:60}
  \begin{align}
    \label{eq:64}
    \vec{v}_k^{+} &=_{\bydefinition} \frac{\vec{w}_k + \vec{w}_{-k}}{2}, \\
    \label{eq:65}
    \vec{v}_k^{-} &=_{\bydefinition} \frac{\vec{w}_k - \vec{w}_{-k}}{2 \iunit}, 
  \end{align}
\end{subequations}
which means that up to an immaterial multiplicative constant we get
\begin{equation}
  \label{eq:69}
  \vec{v}_k^{+} =
  \begin{bmatrix}
    \cos \left( \frac{2 \pi}{n} Nk \right) \\
    \cos \left( \frac{2 \pi}{n} (N-1)k \right) \\
    \vdots \\
    \cos \left( \frac{2 \pi}{n} 2k \right) \\
    \cos \left( \frac{2 \pi}{n} k \right) \\
    \cos \left( \frac{2 \pi}{n} 0 \right) \\
    \cos \left( \frac{2 \pi}{n} k \right) \\
    \cos \left( \frac{2 \pi}{n} 2k \right) \\
    \vdots \\
    \cos \left( \frac{2 \pi}{n} (N-1)k \right) \\
    \cos \left( \frac{2 \pi}{n} Nk \right) 
  \end{bmatrix}
  ,
  \qquad
  \vec{v}_k^{-} =
    \begin{bmatrix}
    \sin \left( \frac{2 \pi}{n} Nk \right) \\
    \sin \left( \frac{2 \pi}{n} (N-1)k \right) \\
    \vdots \\
    \sin \left( \frac{2 \pi}{n} 2k \right) \\
    \sin \left( \frac{2 \pi}{n} k \right) \\
    \sin \left( \frac{2 \pi}{n} 0 \right) \\
    \sin \left( \frac{2 \pi}{n} k \right) \\
    \sin \left( \frac{2 \pi}{n} 2k \right) \\
    \vdots \\
    \sin \left( \frac{2 \pi}{n} (N-1)k \right) \\
    \sin \left( \frac{2 \pi}{n} Nk \right) 
  \end{bmatrix}
  .
\end{equation}
We note that the $m$-th component of the corresponding vector, provided that the elements are indexed from $-N$ to $N$ is given by the formula
\begin{equation}
  \label{eq:70}
  \left(\vec{v}_k^{+}\right)_m = \cos \left( \frac{2 \pi}{n} m k \right) = \cos \left( \frac{2 \pi}{n h} m h  k \right) =  \left. \cos \left( \frac{2 \pi}{n h} x  k \right) \right|_{x = x_m},
\end{equation}
which means that the $m$-th component is obtained via the evaluation/sampling of the function
\begin{equation}
  \label{eq:71}
  \cos \left( \frac{2 \pi}{ \left(2N+1\right) \frac{L}{2N}} x  k \right)
\end{equation}
at the point $x_m = m h$, that is at the point wherein the $m$-th mass is located. This is almost the evaluation/sampling of the $k$-th continuous level eigenfunction $\cos \left(\frac{2 \pi}{L}k x\right)$ at the point $x_m = m h$.
\todo[inline]{It seems that there is $+1$ indexing error somewhere.}

Anyway, the eigenvector are always fine, provided that we deal with a circulant matrix. If we want to recover the behaviour of the continuous operator, all we need to do is to take the \emph{inverse} discrete Fourier transformation of the desired vector of eigenvalues (properly ordered), and we get the first row of the corresponding circulant matrix. This is based on the manipulation in~\eqref{eq:61}.

\todo[inline]{Say why we are not simply doing the following. We want matrix $\tensorq{M}$ with eigenvalues $\left\{\lambda_i\right\}_{i=1}^m$ and (orthonormal) eigenvectors $\left\{\vec{v}_i\right\}_{i=1}^m$, then the matrix is $\tensorq{M} = \sum_{i=1}^m \lambda_i \tensortensor{\vec{v}_i}{\vec{v}_i}$. It is all about interpretation!}

\todo[inline]{Can we interpret the new operator as the discrete convolution/product/whatever of some matrix/vector with the standard second order finite differences differentiation matrix? Something as in~\eqref{eq:45}?}

\endinput

 \section{Continuous representation--subtle issues}
\label{sec:cont-repr}
Now we can try to identify continuous version of~\eqref{eq:118} and~\eqref{eq:123}. The standard case~\eqref{eq:123} is studied in~\cite{huang.hh.sun.ct.ea:on}. A naive continuous limit of~\eqref{eq:123} is based on the finite differences approximation
\begin{equation}
  \label{eq:128}
  \ppd{u}{x} \approx \frac{\uij{1}{j+1} - 2\uij{1}{j} +  \uij{1}{j-1}}{L^2},
\end{equation}
where $h$ denotes the distance between the elementary cells. This brings problems with dispersion relations, see~\cite{challamel.n.zhang.yp.ea:discrete}, \cite{challamel.n.picandet.v.ea:revisiting} and references therein. We can do some nice work here, see the scanned notes.


Concerning the dispersion relation, there are two problems.
\begin{enumerate}
\item We have a discrete system (classical one-dimensional lattice model), and we want to design a continuous system that has the same dispersion relation as the discrete one.
\item We have a continuous system (classical one-dimensional linearised elasticity), and we want to design a discrete lattice system that has the same dispersion relation as the continuous one. 
\end{enumerate}
The problem is not very well defined since the continuous model (partial differential equation) works with an infinite dimensional operator $\ppd{}{x}$, while the lattice model works in the finite dimensional space. 

The dispersion relation for the discrete model is
\begin{equation}
  \label{eq:126}
  \omega^2 = \frac{2 k_1}{m} \left(1 - \cos \left(k L\right) \right),
\end{equation}
where $k$ denotes the wavelength. The corresponding continuous model seems to be
\begin{equation}
  \label{eq:129}
  \rho \ppd{u}{t} + \convolution{g_L}{\ppd{u}{x}} = 0, 
\end{equation}
where
\begin{equation}
  \label{eq:130}
  g_L =_{\bydefinition} \frac{\sqrt{2 \pi} \rho k_1 L}{m} \UnitTriangle \left( \frac{x}{L} \right)
\end{equation}
see the handwritten notes. Note that $g_L$ generates for $L \to \infty$ the delta sequence, hence in the limit $L \to + \infty$ we formally recover the standard linearised elasticity model. Please check!  The approach based on~\eqref{eq:129} is in contrast with the classical approach based on the Taylor expansion of~\eqref{eq:126} as
\begin{equation}
  \label{eq:127}
  \omega^2 = \frac{2 k_1}{m} \left(1 - \cos \left(k L\right) \right) \approx \frac{2 k_1}{m} \left(\frac{k^2L^2}{2!} - \frac{k^4 L^4}{4!} + \cdots \right),
\end{equation}
which leads to continuous models with higher order derivatives, see the standard literature on the subject matter.

On the other hand, the spectrum of $\ppd{}{x}$ is well known, see \href{https://en.wikipedia.org/wiki/Eigenvalues_and_eigenvectors_of_the_second_derivative}{Wikipedia}. We want to design the discrete operator
\begin{equation}
  \label{eq:131}
  \begin{bmatrix}
    c_0 & c_{N-1} & c_{N-2} & c_{N-3} & \dots & c_2 & c_1 \\
    c_1 & c_0 & c_{N-1} & c_{N-2} & \dots & c_3 & c_2 \\
    c_2 & c_1 & c_0 & c_{N-1} & \dots & c_4 & c_3 \\
    \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
    c_{N-2} & c_{N-3} & c_{N-4} & c_{N-5} & \dots & c_0 & c_{N-1} \\
    c_{N-1} & c_{N-2} & c_{N-3} & c_{N-4} & \dots & c_1 & c_0
  \end{bmatrix}
  \begin{bmatrix}
    u_0 \\
    u_1 \\
    u_2 \\
    \vdots \\
    u_{N-2} \\
    u_{N-1}
  \end{bmatrix}
\end{equation}
such that the dispersion relation is the same as the one for continuous problem. (As far as the discrete problem has the sufficient resolving capacity of the continuous eigenfunctions, see the classical aliasing problem.) By the phrase ``design the discrete operator'' we mean the task to identify the constants $c_0$ to $c_N$. The conjecture is described in the handwritten notes. Would it work for multiple frequencies? Note that the matrix in~\eqref{eq:131} is a circulant matrix and everything is known about its eigenvalues and eigenvectors, see \href{https://en.wikipedia.org/wiki/Circulant_matrix}{Wikipedia}, or more seriously \cite{davis.pj:circulant}. Can we interpret~\eqref{eq:131} in terms of long range pairwise interactions?

\section{Miscellaneous}
\label{sec:miscellaneous}

\todo[inline]{Nonlinear oscillators as in \cite{lazarov.bs.jensen.js:low-frequency}?}
\cite{filimonov.am.kurchanov.pf.ea:some,filimonov.am:some}
\cite{andrianov.iv:specific}
\cite{brillouin.l:wave*1}
\cite{kunin.ia:elastic*1,kunin.ia:elastic}

\cite{leveque.rj:finite}
\cite{jovanovic.bs.suli.e:analysis}
\cite{berezovski.a:elastic}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../discrete-versus-continuous"
%%% End:



==> text/miscellaneous.tex <==
\subsection{Alternative approach}
\label{sec:alternative-approach}
We rewrite~\eqref{eq:1} as
\begin{subequations}
  \label{eq:8}
  \begin{align}
    \label{eq:9}
    \ddd{x_1}{t}  + \omega_1^2 \left(1 + \widetilde{k}\right) x_1 - \widetilde{k} \omega_1^2 x_2 & = \frac{f}{m_1}, \\
    \label{eq:10}
    \ddd{x_2}{t}  + \omega_2^2 x_2 - \omega_2^2 x_1 & = 0.
  \end{align}
\end{subequations}
As we have already noted, we are interested in periodic solution of this system. We recall that the (continuous) Fourier transform of $g\colon\, \vec{x} \in \R^n \mapsto \R$ and the corresponding inverse Fourier transform are defined by the formulae
\begin{subequations}
  \label{eq:68}
  \begin{align}
    \label{eq:11}
    \fouriertransform{g(t)}{\omega}
    &=_{\bydefinition}
      \frac{1}{\left(2 \pi \right)^{\frac{1}{2}}}
      \int_{\vec{x} \in \R^n}
      g(t)
      \,
      \exponential{\iunit t \omega}
      \,
      \diff t
      , \\
    \label{eq:12}
    \inversefouriertransform{g(\omega)}{t}
    &=_{\bydefinition}
      \frac{1}{\left(2 \pi \right)^{\frac{1}{2}}}
      \int_{\omega \in \R}
      g(\omega)
      \,
      \exponential{-\iunit t \omega}
      \,
      \diff \omega
      .
  \end{align}
\end{subequations}
Here we use the convention used in~\cite[Theorem 10]{sneddon.in:fourier}. The definition of convolution is then
\begin{equation}
  \label{eq:66}
  (\convolution{f}{g})(x)
  =_{\bydefinition}
  \frac{1}{\sqrt{2 \pi}}
  \int_{y = -\infty}^{+\infty}
  f(x-y)
  g(y)
  \,
  \diff y,
\end{equation}
see~\cite[Section 3.6]{sneddon.in:fourier}, and with this definition of Fourier transform and convolution we obtain the convolution theorem in the form
\begin{equation}
  \label{eq:67}
  \fouriertransform{(\convolution{f}{g})(t)}{\omega}
  =
  \fouriertransform{f(t)}{\omega}
  \fouriertransform{g(t)}{\omega}
  ,
\end{equation}
see~\cite[Theorem 12]{sneddon.in:fourier}.


The Fourier transformed version of~\eqref{eq:8} reads
\begin{subequations}
  \label{eq:14}
  \begin{align}
    \label{eq:15}
    - \omega^2 \FourierTransform{x_1}  + \omega_1^2 \left(1 + \widetilde{k}\right) \FourierTransform{x_1} - \widetilde{k} \omega_1^2 \FourierTransform{x_2} & = \frac{1}{m_1} \FourierTransform{f}, \\
    \label{eq:16}
    - \omega^2 \FourierTransform{x_2}  + \omega_2^2 \FourierTransform{x_2} - \omega_2^2 \FourierTransform{x_1} & = 0.
  \end{align}
\end{subequations}
This system is converted into the matrix form as
\begin{equation}
  \label{eq:17}
  \left(
    -
    \omega^2
    \begin{bmatrix}
      1 & 0 \\
      0 & 1
    \end{bmatrix}
    +
    \begin{bmatrix}
      \omega_1^2 \left(1 + \widetilde{k}\right) & - \widetilde{k} \omega_1^2 \\
      - \omega_2^2 & \omega_2^2 
    \end{bmatrix}
  \right)
  \begin{bmatrix}
    \FourierTransform{x_1} \\
    \FourierTransform{x_2}
  \end{bmatrix}
  =
  \begin{bmatrix}
    \frac{1}{m_1} \FourierTransform{f} \\
    0
  \end{bmatrix}
  ,
\end{equation}
and if we define the matrix $\tensorq{M}$ (mass matrix) and the matrix $\tensorq{K}$ (stiffness matrix) as 
\begin{subequations}
  \label{eq:62}
  \begin{align}
    \label{eq:63}
    \tensorq{M} & =_\bydefinition
                  \begin{bmatrix}
                    1 & 0 \\
                    0 & 1
                  \end{bmatrix},
    \\
    \label{eq:64}
    \tensorq{K} & =_\bydefinition
                  \begin{bmatrix}
                    \omega_1^2 \left(1 + \widetilde{k}\right) & - \widetilde{k} \omega_1^2 \\
                    - \omega_2^2 & \omega_2^2 
                  \end{bmatrix}
                  ,
  \end{align}
\end{subequations}
then we can rewrite the system in the compact form as
\begin{equation}
  \label{eq:65}
  \left(
    -
    \omega^2 \tensorq{M}
    +
    \tensorq{K}
  \right)
  \FourierTransform{\vec{x}}
  =
  \FourierTransform{\frac{\vec{f}}{m_1}}
  .
\end{equation}
The matrix
\begin{equation}
  \label{eq:18}
  \tensorq{A} =_{\bydefinition}
  -
  \omega^2 \tensorq{M}
  +
  \tensorq{K}
\end{equation}
is diagonalised by the similarity transformation
\begin{equation}
  \label{eq:19}
  \tensorq{A}
  =
  \tensorq{C}
  \tensorq{J}
  \inverse{
    \tensorq{C}
  },
\end{equation}
wherein the diagonal matrix $\tensorq{J}$ is given by the formula
\begin{equation}
  \label{eq:21}
  \tensorq{J}
  =
  \begin{bmatrix}
    \frac{1}{2}
    \left(a^2 - b^2\right) - \omega^2 & 0 \\
    0 & \frac{1}{2} \left(a^2 + b^2\right) - \omega^2
  \end{bmatrix}
  ,
\end{equation}
with
\begin{subequations}
  \label{eq:23}
  \begin{align}
    \label{eq:24}
    a^2 &=_{\bydefinition}  \omega_1^2 \left(\widetilde{k}+1\right) + \omega_2^2, \\
    \label{eq:25}
    b^2 &=_{\bydefinition} \sqrt{ \omega_1^4 \left(\widetilde{k}+1\right)^2 + 2 \omega_1^2 \omega_2^2\left(\widetilde{k}+1\right) + \omega_2^4}. 
  \end{align}
\end{subequations}
(See below for an explicit formula for the similarity transformation matrix $\tensorq{C}$.) We note that the term under the square root in~\eqref{eq:25} can be rewritten either as
\begin{equation}
  \label{eq:26}
  \omega_1^4 \left(\widetilde{k}+1\right)^2 + 2 \omega_1^2 \omega_2^2\left(\widetilde{k}+1\right) + \omega_2^4
  =
  \left(
    \omega_1^2 \left(\widetilde{k}+1\right) + \omega_2^2
  \right)^2
  -
  4 \omega_1^2 \omega_2^2
\end{equation}
or
\begin{equation}
  \label{eq:27}
  \omega_1^4 \left(\widetilde{k}+1\right)^2 + 2 \omega_1^2 \omega_2^2\left(\widetilde{k}+1\right) + \omega_2^4
  =
  \left(
    \omega_1^2 \left(\widetilde{k}+1\right) - \omega_2^2
  \right)^2
  +
  4 \omega_1^2 \omega_2^2 \widetilde{k}.
\end{equation}
The latter form~\eqref{eq:27} reveals that the term under square root in~\eqref{eq:25} is positive, while the former form~\eqref{eq:26} allows us to rewrite~\eqref{eq:25} as
\begin{equation}
  \label{eq:28}
  b^2 = \sqrt{a^4 -  4 \omega_1^2 \omega_2^2}.
\end{equation}
Finally, we denote
\begin{subequations}
  \label{eq:31}
  \begin{align}
    \label{eq:32}
    c_1^2 &=_{\bydefinition} \frac{1}{2} \left( a^2 - b^2 \right), \\
    \label{eq:33}
    c_2^2 &=_{\bydefinition} \frac{1}{2} \left( a^2 + b^2 \right),
  \end{align}
\end{subequations}
and in virtue of~\eqref{eq:28} we see that $c_1^2$ is indeed positive, and that the formula for the diagonal matrix $\tensorq{J}$ simplifies to
\begin{equation}
  \label{eq:30}
  \tensorq{J}
  =
  \begin{bmatrix}
    c_1^2 - \omega^2 & 0 \\
    0 & c_2^2 - \omega^2
  \end{bmatrix}
  .
\end{equation}
The formula for the similarity transformation matrix reads
\begin{equation}
  \label{eq:20}
  \tensorq{C}
  =
  \begin{bmatrix}
    \frac{e + b^2}{2 \omega_2^2}
    &
      \frac{e - b^2}{2 \omega_2^2}
    \\
    1 & 1
  \end{bmatrix}
\end{equation}
with
\begin{equation}
  \label{eq:37}
  \inverse{\tensorq{C}}
  =
  \begin{bmatrix}
    \frac{\omega_2^2}{b^2}
    &
      -\frac{e - b^2}{2 b^2}
    \\
    -\frac{\omega_2^2}{b^2}
    &
      \frac{e + b^2}{2 b^2}
  \end{bmatrix}
\end{equation}
where
\begin{equation}
  \label{eq:35}
  e =_{\bydefinition} - \omega_1^2 \left(\widetilde{k}+1\right) + \omega_2^2.
\end{equation}
We note that the columns of matrix $\tensorq{C}$ are \emph{not} mutually orthogonal, indeed
\begin{equation}
  \label{eq:36}
  \vectordot{
    \begin{bmatrix}
      \frac{e + b^2}{2 \omega_2^2}
      \\
      1
    \end{bmatrix}
  }
  {
    \begin{bmatrix}
      \frac{e - b^2}{2 \omega_2^2}
      \\
      1
    \end{bmatrix}
  }
  =
  \frac{e^2 - b^4}{4 \omega_2^4}
  +
  1
  =
  \frac{
    \left( \omega_1^2 \left(\widetilde{k}+1\right) - \omega_2^2 \right)^2
    -
    \left(
      \omega_1^2 \left(\widetilde{k}+1\right) - \omega_2^2
    \right)^2
    -
    4 \omega_1^2 \omega_2^2 \widetilde{k}
  }
  {
    4 \omega_2^4
  }
  +
  1
  =
  1
  -
  \frac{\omega_1^2}{\omega_2^2} \widetilde{k}.
\end{equation}
This means that the eigenvectors of $\tensorq{A}$ are not orthogonal.

Using the transformation matrix $\tensorq{C}$, we see that the equation
\begin{equation}
  \label{eq:38}
  \tensorq{A}
  \begin{bmatrix}
    \FourierTransform{x_1} \\
    \FourierTransform{x_2}
  \end{bmatrix}
  =
  \begin{bmatrix}
    \frac{1}{m_1} \FourierTransform{f} \\
    0
  \end{bmatrix}
\end{equation}
can be rewritten as
\begin{equation}
  \label{eq:39}
  \tensorq{C}
  \tensorq{J}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \FourierTransform{x_1} \\
    \FourierTransform{x_2}
  \end{bmatrix}
  =
  \begin{bmatrix}
    \frac{1}{m_1} \FourierTransform{f} \\
    0
  \end{bmatrix}
  ,
\end{equation}
which reduces to
\begin{equation}
  \label{eq:40}
  \tensorq{J}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \FourierTransform{x_1} \\
    \FourierTransform{x_2}
  \end{bmatrix}
  =
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \frac{1}{m_1} \FourierTransform{f} \\
    0
  \end{bmatrix}
  .
\end{equation}
We denote
\begin{equation}
  \label{eq:41}
  \FourierTransform{\vec{z}} =_{\bydefinition}  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \FourierTransform{x_1} \\
    \FourierTransform{x_2}
  \end{bmatrix}
\end{equation}
and we see that~\eqref{eq:40} reduces to
\begin{equation}
  \label{eq:13}
  \tensorq{J}
  \FourierTransform{\vec{z}}
  =
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \frac{1}{m_1} \FourierTransform{f} \\
    0
  \end{bmatrix},
\end{equation}
which is easy to solve
\begin{equation}
  \label{eq:22}
  \FourierTransform{\vec{z}}
  =
  \inverse{\tensorq{J}}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \frac{1}{m_1} \FourierTransform{f} \\
    0
  \end{bmatrix}
  .
\end{equation}
If the right-hand side has the form $f = \widehat{F} \sin \left(\Omega t\right)$, then
\begin{equation}
  \label{eq:29}
  \FourierTransform{f}
  =
  \iunit
  \sqrt{\frac{\pi}{2}}
  \widehat{F}
  \left(
    \diracdelta\left(\omega - \Omega \right)
    -
    \diracdelta\left(\omega + \Omega \right)
  \right)
\end{equation}
where $\diracdelta$ denotes the Dirac delta function, and~\eqref{eq:22} reduces to
\begin{equation}
  \label{eq:34}
  \FourierTransform{\vec{z}}
  =
  \iunit
  \sqrt{\frac{\pi}{2}}
  \begin{bmatrix}
    \frac{ \diracdelta\left(\omega - \Omega \right) - \diracdelta\left(\omega + \Omega \right)}{c_1^2 - \omega^2} & 0 \\
    0 & \frac{ \diracdelta\left(\omega - \Omega \right) - \diracdelta\left(\omega + \Omega \right)}{c_2^2 - \omega^2}
  \end{bmatrix}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \frac{\widehat{F}}{m_1}\\
    0
  \end{bmatrix}
  ,
\end{equation}
and by the linearity of the Fourier transformation we get
\begin{equation}
  \label{eq:42}
  \begin{bmatrix}
    x_1 \\
    x_2
  \end{bmatrix}
  =
  \tensorq{C}
  \begin{bmatrix}
    \InverseFourierTransform{\iunit \sqrt{\frac{\pi}{2}} \frac{ \diracdelta\left(\omega - \Omega \right) - \diracdelta\left(\omega + \Omega \right)}{c_1^2 - \omega^2}} & 0 \\
    0 &   \InverseFourierTransform{\iunit \sqrt{\frac{\pi}{2}} \frac{ \diracdelta\left(\omega - \Omega \right) - \diracdelta\left(\omega + \Omega \right)}{c_2^2 - \omega^2}}
  \end{bmatrix}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \frac{\widehat{F}}{m_1}\\
    0
  \end{bmatrix}
  ,
\end{equation}
which yields
\begin{equation}
  \label{eq:43}
  \begin{bmatrix}
    x_1 \\
    x_2
  \end{bmatrix}
  =
  \tensorq{C}
  \begin{bmatrix}
    \frac{\sin \left(\Omega t \right)}{c_1^2 - \Omega^2} & 0 \\
    0 &  \frac{\sin \left(\Omega t \right)}{c_2^2 - \Omega^2}
  \end{bmatrix}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    \frac{\widehat{F}}{m_1}\\
    0
  \end{bmatrix}
\end{equation}
or
\begin{equation}
  \begin{bmatrix}
    x_1 \\
    x_2
  \end{bmatrix}
  =
  \tensorq{C}
  \begin{bmatrix}
    \frac{1}{c_1^2 - \Omega^2} & 0 \\
    0 &  \frac{1}{c_2^2 - \Omega^2}
  \end{bmatrix}
  \inverse{\tensorq{C}}
  \begin{bmatrix}
    1\\
    0
  \end{bmatrix}
  \frac{\widehat{F}}{m_1}
  \sin \left(\Omega t \right),
\end{equation}
or
\begin{equation}
  \label{eq:45}
  x_2
  =
  \left(
    \vectordot{
      \begin{bmatrix}
        0\\
        1
      \end{bmatrix}
    }
    {
      \left(
        \tensorq{C}
        \begin{bmatrix}
          \frac{1}{c_1^2 - \Omega^2} & 0 \\
          0 &  \frac{1}{c_2^2 - \Omega^2}
        \end{bmatrix}
        \inverse{\tensorq{C}}
        \begin{bmatrix}
          1\\
          0
        \end{bmatrix}
      \right)
    }
  \right)
  \frac{\widehat{F}}{m_1}
  \sin \left(\Omega t \right)
  .
\end{equation}
Using the explicit formulae for the transformation matrix $\tensorq{C}$, we see that the last formula simplifies to
\begin{multline}
  \label{eq:46}
  x_2
  =
  \left(
    \vectordot{
      \begin{bmatrix}
        0\\
        1
      \end{bmatrix}
    }
    {
      \left(
        \tensorq{C}
        \begin{bmatrix}
          \frac{1}{c_1^2 - \Omega^2} & 0 \\
          0 &  \frac{1}{c_2^2 - \Omega^2}
        \end{bmatrix}
        \inverse{\tensorq{C}}
        \begin{bmatrix}
          1\\
          0
        \end{bmatrix}
      \right)
    }
  \right)
  \frac{\widehat{F}}{m_1}
  \sin \left(\Omega t \right)
  =
  \left(
    \vectordot{
      \begin{bmatrix}
        0\\
        1
      \end{bmatrix}
    }
    {
      \left(
        \tensorq{C}
        \begin{bmatrix}
          \frac{1}{c_1^2 - \Omega^2} & 0 \\
          0 &  \frac{1}{c_2^2 - \Omega^2}
        \end{bmatrix}
        \begin{bmatrix}
          1\\
          -1
        \end{bmatrix}
      \right)
    }
  \right)
  \frac{\omega_2^2}{b^2}
  \frac{\widehat{F}}{m_1}
  \sin \left(\Omega t \right)
  \\
  =
  \left(
    \vectordot{
      \begin{bmatrix}
        0\\
        1
      \end{bmatrix}
    }
    {
      \left(
        \tensorq{C}
        \begin{bmatrix}
          \frac{1}{c_1^2 - \Omega^2}\\
          -\frac{1}{c_2^2 - \Omega^2}
        \end{bmatrix}
      \right)
    }
  \right)
  \frac{\omega_2^2}{b^2}
  \frac{\widehat{F}}{m_1}
  \sin \left(\Omega t \right)
  =
  \left(
    \frac{1}{c_1^2 - \Omega^2}
    -
    \frac{1}{c_2^2 - \Omega^2}
  \right)
  \frac{\omega_2^2}{b^2}
  \frac{\widehat{F}}{m_1}
  \sin \left(\Omega t \right).
\end{multline}
Since we now have an explicit solution for $x_2$ we can use it in~\eqref{eq:2} and rewrite~\eqref{eq:2} as
\begin{equation}
  \label{eq:47}
  m_1 \ddd{x_1}{t}  + \left(k_1 + k_2 \right) x_1
  =
  \left(1 + \frac{k_2}{m_1}
    \left(
      \frac{1}{c_1^2 - \Omega^2}
      -
      \frac{1}{c_2^2 - \Omega^2}
    \right)
    \frac{\omega_2^2}{b^2}
  \right)
  \widehat{F}\sin \left( \Omega t \right)
  ,
\end{equation}
which can be further rewritten as
\begin{equation}
  \label{eq:48}
  m_1 \ddd{x_1}{t}  + k_1\left(1 + \widetilde{k} \right) x_1
  =
  \left(
    1
    +
    \widetilde{k} 
    \frac{\omega_1^2\omega_2^2}{b^2}
    \left(
      \frac{1}{c_1^2 - \Omega^2}
      -
      \frac{1}{c_2^2 - \Omega^2}
    \right)
  \right)
  \widehat{F}\sin \left( \Omega t \right)
  .
\end{equation}
\emph{We have been studying only particular solution!} In this sense we see that we can forget everything about the second body, and treat the system as one degree-of-freedom system with mass $m_1$, stiffness $k_1\left(1 + \widetilde{k} \right)$ and force with the amplitude modulated by a scalar factor. There is no need to introduce the negative mass.

Note that we could have also used
\begin{multline}
  \label{eq:44}
  \InverseFourierTransform{\iunit \sqrt{\frac{\pi}{2}} \frac{ \diracdelta\left(\omega - \Omega \right) - \diracdelta\left(\omega + \Omega \right)}{c_1^2 - \omega^2}}
  =
  \InverseFourierTransform{ \frac{1}{c_1^2 - \omega^2} \FourierTransform{\sin \left(\Omega t\right)}}
  \\
  =
  \InverseFourierTransform{ \FourierTransform{\sqrt{\frac{\pi}{2}} \signum(t) \frac{\sin \left(c_1 t\right)}{c_1}} \FourierTransform{\sin \left(\Omega t\right)}}
  =
  \InverseFourierTransform{\sqrt{\frac{\pi}{2}} \FourierTransform{\convolution{\signum(t) \frac{\sin \left(c_1 t\right)}{c_1}}{\sin \left(\Omega t\right)}}}
  \\
  =
  \sqrt{\frac{\pi}{2}} \convolution{\signum(t) \frac{\sin \left(c_1 t\right)}{c_1}}{\sin \left(\Omega t\right)}.
\end{multline}


